Science, AskScience, and BadScience: On the Coexistence of Highly Related Communities

When large social-media platforms allow users to easily form and self-organize into interest groups, highly related communities can arise. For example, the Reddit site hosts not just a group called food, but also HealthyFood, foodhacks, foodporn, and cooking, among others. Are these highly related communities created for similar classes of reasons (e.g., to focus on a subtopic, to create a place for allegedly more "high-minded" discourse, etc.)? How do users allocate attention between such close alternatives when they are available or emerge over time? Are there different types of relations between close alternatives such as sharing many users vs. a new community drawing away members of an older one vs. a splinter group failing to cohere into a viable separate community? We investigate the interactions between highly related communities using data from reddit.com consisting of 975M posts and comments spanning an 8-year period. We identify a set of typical affixes that users adopt to create highly related communities and build a taxonomy of affixes. One interesting finding regarding users' behavior is: after a newer community is created, for several types of highly-related community pairs, users that engage in a newer community tend to be more active in their original community than users that do not explore, even when controlling for previous level of engagement.

==> figures/exploration/modification_table.tex <==
\modifier{s} & \communityname{auto}, \communityname{autos} & 63 \\
\modifier{porn} & \communityname{space}, \communityname{spaceporn} & 26  \\
\modifier{circlejerk} & \communityname{hiphop}, \communityname{hiphopcirclejerk} & 23 \\
\modifier{ask} & \communityname{science}, \communityname{askscience} & 21 \\
\modifier{shitty} & \communityname{ideas}, \communityname{shittyideas} & 17 \\
\modifier{music} & \communityname{running}, \communityname{runningmusic} & 17 \\
\modifier{help} & \communityname{tech}, \communityname{techhelp} & 11\\
\modifier{2} & \communityname{dota}, \communityname{dota2} & 9\\
\modifier{true} & \communityname{atheism}, \communityname{trueatheism} & 9 \\
\modifier{learn} & \communityname{math}, \communityname{learnmath} & 9\\


==> figures/exploration/taxonomy.tex <==
\begin{tabular}{p{0.8in}p{2.2in}} 
\toprule
\multicolumn{2}{c}{Adjective-like}\\
\midrule
``better'' & true, plus\\
``parody'' & circlejerk, shitty, funny, lol, bad\\
``derivative'' & post, ex, meta, anti, srs \\
``genre'' & classic, fantasy, indie, folk, casual, dirty, classic, metal, academic, 90s, free, social\\
``nsfw'' & nsfw\_, nsfw, asian, trees, gonewild, gw, r4r, tree\\
\midrule
\multicolumn{2}{c}{Verb-like}\\
\midrule
``learning, improvement'' & ask, help, learn, advice, hacks, stop\\
``action'' & exchange, randomactsof, trade, trades, classifieds, market, swap, random\_acts\_of\_, requests, invites, builds, making, mining, craft\\
\midrule
\multicolumn{2}{c}{Noun-like}\\
\midrule
``place'' & uk, reddit, chicago, us, dc, steam, canada, american, boston, android, online, web\\
``medium'' & porn, pics, music, memes, videos, vids, comics, apps, games, gaming, game\\
``subject'' & science, news, dev, servers, tech,  tv, guns, recipes, city, u, college, man, girls\\
\midrule
\multicolumn{2}{c}{Minor}\\
\midrule
``equivalent, competition'' & s, al, ing, the, alternative\\
``generation'' & 2, 3, 4, 5 \\
``modifier'' & ism, n, an\\
% minor (84) & s, ism, al, n, an, ing, the\\
% number (21) & 2, 3, 4, 5 \\
% verb (33) & ask, learn, stop\\
% adjective (149) & shitty, true, funny, post, randomactsof, lol, nsfw\_, bad, online, web, meta, srs, social, plus, asian, alternative, casual, free, indie, nsfw, dirty, classic, metal, academic, tech, random\_acts\_of\_, ex, folk, 90s, american, anti\\
% noun (285) & porn, circlejerk, help, music, trees, news, pics, memes, games, videos, advice, game, exchange, trade, uk, reddit, chicago, u, dev, gaming, gw, vids, trades, servers, fantasy, classifieds, market, r4r, gonewild, builds, science, us, tv, swap, dc, steam, hacks, college, canada, guns, recipes, requests, invites, apps, city, girls, mining, craft, comics, tree, making, boston, android, man\\
% \midrule
% \multicolumn{2}{c}{Community Function Classification} \\
%%JMH-01-10: Added quotes around these to distinguish them from modifications
% (jokes, antijokes, antiantijokes, 5anti)
\bottomrule
\end{tabular}
